The Analysis of Online Event Streams: Predicting the Next Activity for Anomaly Detection

Anomaly detection in process mining focuses on identifying anomalous cases or events in process executions. The resulting diagnostics are used to provide measures to prevent fraudulent behavior, as well as to derive recommendations for improving process compliance and security. Most existing techniques focus on detecting anomalous cases in an offline setting. However, to identify potential anomalies in a timely manner and take immediate countermeasures, it is necessary to detect event-level anomalies online, in real-time. In this paper, we propose to tackle the online event anomaly detection problem using next-activity prediction methods. More specifically, we investigate the use of both ML models (such as RF and XGBoost) and deep models (such as LSTM) to predict the probabilities of next-activities and consider the events predicted unlikely as anomalies. We compare these predictive anomaly detection methods to four classical unsupervised anomaly detection approaches (such as Isolation forest and LOF) in the online setting. Our evaluation shows that the proposed method using ML models tends to outperform the one using a deep model, while both methods outperform the classical unsupervised approaches in detecting anomalous events.

==> backup.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccc}
\hline
 & \textbf{Online/ Offline} & \textbf{Target status} & \textbf{Algorithm} \\ \hline
Ghionna et al.~\cite{ghionna2008outlier} & \multirow{6}{*}{Offline} & \multirow{3}{*}{Case} & Markov cluster \\ \cline{1-1} \cline{4-4} 
Sani et al.~\cite{sani2017improving} &  &  & Occurance proability \\ \cline{1-1} \cline{4-4} 
Khatuya et al.~\cite{khatuya2018adele} &  &  & Ridge regression \\ \cline{1-1} \cline{3-4} 
Nguyen et al.~\cite{nguyen2019autoencoders} &  & \multirow{3}{*}{Event} & Autoencoder \\ \cline{1-1} \cline{4-4} 
Savickas and Vasilecas~\cite{savickas2018belief} &  &  & Bayesian belief network \\ \cline{1-1} \cline{4-4} 
Nolle et al.~\cite{nolle2022binet} &  &  & LSTM \\ \hline
Tavares et al.~\cite{tavares2019overlapping} & \multirow{5}{*}{Online} & \multirow{3}{*}{Case} & Process model conformity check \\ \cline{1-1} \cline{4-4} 
Ko and Comuzzi~\cite{ko2020online} &  &  & Leverage score calculation \\ \cline{1-1} \cline{4-4} 
Neto et al.~\cite{vertuam2021use} &  &  & Autocloud \\ \cline{1-1} \cline{3-4} 
Van Zelst et al.~\cite{van2018filtering} &  & \multirow{2}{*}{Event} & Automaton processor \\ \cline{1-1} \cline{4-4} 
Krajsic and Franczyk~\cite{krajsic2020lambda} &  &  & Autoencoder \\ \hline
\end{tabular}%
}
\caption{Comparison of related anomaly detection approaches}
\label{tab:related_works_table}
\end{table}

==> files/research_challenge.tex <==
As a relatively new research area, anomalous event detection in even streams has open challenges in several perspectives. We identifies multiple challenges on online anomaly detection that are needed to be answered.

\begin{enumerate}[label=]%[label=\textbf{RQ{\arabic*}}]
    \item \RQ{RQ1}{We don't know anomalies is definite}
    \item \RQ{RQ2}{How can we guarantee on case termination in a streaming event log?} \xixi{What do you mean with case initialization and termination?}
    \item \RQ{RQ3}{How can anomalies in an event log can be detected taking into account concept drift occurrence?}
    \xixi{It is a nice challenge but did your approach solve this? And do you have evidence that you approach solves this challenge?}
    % \item \RQ{RQ3}{When can the process user reacts anomalies from the executed events?}
    % \xixi{The same as above}
\end{enumerate}

This paper focuses on the solutions for the last two challenges by actively reacting to incoming events and notifying the detected anomalous events to the process user just in time. 

% In~\cite{van2019process}, research directions are proposed for applying process mining with streaming event data. With addressed directions, 
